Online Convex Optimization with Switching Cost and Delayed Gradients

We consider the online convex optimization (OCO) problem with quadratic and linear switching cost in the limited information setting, where an online algorithm can choose its action using only gradient information about the previous objective function. For $L$-smooth and $\mu$-strongly convex objective functions, we propose an online multiple gradient descent (OMGD) algorithm and show that its competitive ratio for the OCO problem with quadratic switching cost is at most $4(L + 5) + \frac{16(L + 5)}{\mu}$. The competitive ratio upper bound for OMGD is also shown to be order-wise tight in terms of $L,\mu$. In addition, we show that the competitive ratio of any online algorithm is $\max\{\Omega(L), \Omega(\frac{L}{\sqrt{\mu}})\}$ in the limited information setting when the switching cost is quadratic. We also show that the OMGD algorithm achieves the optimal (order-wise) dynamic regret in the limited information setting. For the linear switching cost, the competitive ratio upper bound of the OMGD algorithm is shown to depend on both the path length and the squared path length of the problem instance, in addition to $L, \mu$, and is shown to be order-wise, the best competitive ratio any online algorithm can achieve. Consequently, we conclude that the optimal competitive ratio for the quadratic and linear switching costs are fundamentally different in the limited information setting.

==> Proof_lemma_lb_linear.tex <==
\section{Proof of Lemma \ref{lem:lb_linear}}\label{app:lb_linear}
	Consider the sequence of functions given by \(f_{t}(x_{t}) = \frac{\mu}{2} (x_{t} - v_{t}) ^ {2}\), where the sequence \(v_{1}, \dots, v_{T}\) satisfies the following \begin{align}
		v_{T} - \frac{1}{\mu} \geq v_{T - 1} \geq v_{T - 2} \geq \dots \geq v_{2} \geq v_{1} \geq 0\nn
	\end{align}
	A lower bound on \(C_{\opt}\) can be obtained in the following manner:
	\begin{align}
		C_{\opt}
		& = \sum_{t = 1} ^ {T} \big(\frac{\mu}{2}(x_{t} - v_{t}) ^ {2} + \abs{x_{t} - x_{t - 1}}\big),\nn \\
		& \stackrel{(a)}\geq \sum_{t = 1} ^ {T} \big(\frac{\mu}{2}(x_{t} - v_{t}) ^ {2} + x_{t} - x_{t - 1}\big),\nn \\
		& \stackrel{(b)}= v_{T} - \frac{1}{2\mu},\nn
	\end{align}
	where \((a)\) follows by the trivial inequality \(\abs{x} \geq x\) and \((b)\) follows by solving the minimization \(\min_{x_{T}} \big(\frac{\mu}{2}(x_{T} - v_{T}) ^ {2} + v_{T}\big)\). Since \(v_{T} - v_{ T - 1} \geq \frac{1}{\mu}\) we have \(C_{\opt} \geq \frac{v_{T} + v_{T - 1}}{2} = \frac{v_{T} - v_{T - 1}}{2} + (v_{T - 1} - v_{T - 2}) + \dots + (v_{2} - v_{1}) + v_{1} \geq \frac{\cP_{T}^\star + \abs{v_{1}}}{2}\). This completes the proof.

==> input.tex <==
\usepackage{fancyhdr}
\pagestyle{fancy}
%\usepackage[printwatermark]{xwatermark}
%\usepackage{xcolor}
%\usepackage{lipsum}
%\usepackage{graphicx}
%\usepackage[a6paper]{geometry}
%\usepackage{draftwatermark}
\usepackage{url}
%\usepackage{lipsum}

\usepackage{amsfonts}
\usepackage{times}
%\usepackage[pdftex]{graphicx}
%\usepackage{mathtools}
%\usepackage[dvips]{graphics}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
\usepackage{tikz}
\usetikzlibrary{math}
\usepackage{listofitems}
\catcode`\_11
\def\reassignitem#1[#2]#3{\loi_argcsname\loi_def{\loi_macroname#1[#2]}{#3}}
\loi_restorecatcode

\usetikzlibrary{decorations.text,calc,arrows.meta}
\usepackage{pgfplots}
\usetikzlibrary {positioning}
\usetikzlibrary{shapes,snakes}
\usetikzlibrary{arrows,calc}
\usepackage{relsize}
\usetikzlibrary{patterns}
\usepackage{enumitem}

%\usepackage[margin=15mm]{geometry}

\usepackage{arrayjobx}
\usepackage{trimspaces}

    \makeatletter
    \def\trimspace#1{\trim@spaces@in{#1}}
    \makeatother
\usepackage{tcolorbox}

\usepackage{longtable}
\usepackage{lipsum}
%\DeclareGraphicsExtensions{.jpg}
%\usepackage[dvips]{graphicx}
%\DeclareGraphicsExtensions{.eps}
%\usepackage{dsfont}
%\usepackage[T1]{fontenc}
%\usepackage[utf8]{inputenc}
%\usepackage{babel}
%\usepackage{appendix}
%\usepackage{blindtext}

\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{cite}
\usepackage{verbatim}
\usepackage{braket}
\usepackage{subfigure}
\newtheorem{thm}{Theorem}[section]
%\newtheorem{definition}{Definition}[section]
\usepackage{epsfig}
 \usepackage{epstopdf}
 \usepackage{psfrag}
 \usepackage{color}
\epstopdfsetup{outdir=./}
\graphicspath{{../}}
 
 \usepackage{subfigure}
%\usepackage{eps}
\usepackage{amsmath,amssymb}
%\usepackage{graphicx}
\usepackage{color}
\usepackage{cite}
\usepackage{multirow,tabularx}
\usepackage{ifthen}
% Add these after the document class declaration
\usepackage{times}
%\usepackage{graphicx}
\usepackage{amsbsy} 
\usepackage{epsfig}
\usepackage{color}
%\usepackage{epstoeps}

\DeclareGraphicsRule{.pstex}{eps}{*}{}
 \DeclareGraphicsRule{.epstex}{pdf}{*}{}

\usepackage{stackrel}


\usepackage{amsfonts}
\usepackage{stfloats}
\usepackage{float}
\usepackage[all]{xy}

 
\DeclareGraphicsRule{.pstex}{eps}{*}{}
 \DeclareGraphicsRule{.epstex}{pdf}{*}{}

\usepackage{makeidx} %originally not
\makeindex %originally not

\newcommand{\marceau}[1]{\color{black}#1\color{black}}

\newcommand\smallO{
  \mathchoice
    {{\scriptstyle\mathcal{O}}}% \displaystyle
    {{\scriptstyle\mathcal{O}}}% \textstyle
    {{\scriptscriptstyle\mathcal{O}}}% \scriptstyle
    {\scalebox{.7}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
  }

\newtheorem{acknowledgement}[thm]{Acknowledgement}
%\newtheorem{algorithm}[thm]{Algorithm}
%\newtheorem{assumption}[thm]{Assumption}
%\newtheorem{axiom}[thm]{Axiom}
\newtheorem{case}[thm]{Case}
\newtheorem{claim}[thm]{Claim}
\newtheorem{conclusion}[thm]{Conclusion}
\newtheorem{condition}[thm]{Condition}
%\newtheorem{conjecture}[thm]{Conjecture}
%\newtheorem{corollary}[thm]{Corollary}
\newtheorem{criterion}[thm]{Criterion}
%\newtheorem{defn}[thm]{Definition}
%\newtheorem{example}[definition]{Example}
\newtheorem{exercise}[thm]{Exercise}
\newtheorem{fact}[thm]{Fact}
%\newtheorem{lemma}[thm]{Lemma}
\newtheorem{notation}[thm]{Notation}
\newtheorem{problem}[thm]{Problem}
\newtheorem{prop}[thm]{Proposition}
%\newtheorem{solution}[thm]{Solution}
\newtheorem{summary}[thm]{Summary}
%\newtheorem{remark}[thm]{Remark}
%\newtheorem{rem}[thm]{Remark}

\newcommand{\Example}[1]{
{
\begin{tcolorbox}
\begin{quote}
#1
\end{quote}
\end{tcolorbox}
}}


%\newenvironment{proof}{ \textbf{Proof:} }{ \hfill $\Box$}
\newenvironment{soln}{ \textbf{Solution:} }{ \hfill $\Box$}


\newcommand{\figref}[1]{{Fig.}~\ref{#1}}
\newcommand{\tabref}[1]{{Table}~\ref{#1}}
\newcommand{\bookemph}[1]{ {\em #1}}
\newcommand{\Ns}{N_s}
\newcommand{\Ut}{U_t}
\newcommand{\fig}[1]{Fig.\ \ref{#1}}
\def\onehalf{\frac{1}{2}}
\def\etal{et.\/ al.\/}
\newcommand{\bydef}{\triangleq}
\newcommand{\tr}{tr}


% blackboard lowercase
\def\bydef{:=}
\def\bba{{\mathbb{a}}}
\def\bbb{{\mathbb{b}}}
\def\bbc{{\mathbb{c}}}
\def\bbd{{\mathbb{d}}}
\def\bbee{{\mathbb{e}}}
\def\bbff{{\mathbb{f}}}
\def\bbg{{\mathbb{g}}}
\def\bbh{{\mathbb{h}}}
\def\bbi{{\mathbb{i}}}
\def\bbj{{\mathbb{j}}}
\def\bbk{{\mathbb{k}}}
\def\bbl{{\mathbb{l}}}
\def\bbm{{\mathbb{m}}}
\def\bbn{{\mathbb{n}}}
\def\bbo{{\mathbb{o}}}
\def\bbp{{\mathbb{p}}}
\def\bbq{{\mathbb{q}}}
\def\bbr{{\mathbb{r}}}
\def\bbs{{\mathbb{s}}}
\def\bbt{{\mathbb{t}}}
\def\bbu{{\mathbb{u}}}
\def\bbv{{\mathbb{v}}}
\def\bbw{{\mathbb{w}}}
\def\bbx{{\mathbb{x}}}
\def\bby{{\mathbb{y}}}
\def\bbz{{\mathbb{z}}}
\def\bb0{{\mathbb{0}}}
%\def\b1{{\mathbf{1}}}
\def\b1{{\mathbf{1}}}

% Bold lowercase
\def\bydef{:=}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
%\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\b0{{\mathbf{0}}}

% Bold capital letters
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

% Blackboard capital letters
\def\bbA{{\mathbb{A}}}
\def\bbB{{\mathbb{B}}}
\def\bbC{{\mathbb{C}}}
\def\bbD{{\mathbb{D}}}
\def\bbE{{\mathbb{E}}}
\def\bbF{{\mathbb{F}}}
\def\bbG{{\mathbb{G}}}
\def\bbH{{\mathbb{H}}}
\def\bbI{{\mathbb{I}}}
\def\bbJ{{\mathbb{J}}}
\def\bbK{{\mathbb{K}}}
\def\bbL{{\mathbb{L}}}
\def\bbM{{\mathbb{M}}}
\def\bbN{{\mathbb{N}}}
\def\bbO{{\mathbb{O}}}
\def\bbP{{\mathbb{P}}}
\def\bbQ{{\mathbb{Q}}}
\def\bbR{{\mathbb{R}}}
\def\bbS{{\mathbb{S}}}
\def\bbT{{\mathbb{T}}}
\def\bbU{{\mathbb{U}}}
\def\bbV{{\mathbb{V}}}
\def\bbW{{\mathbb{W}}}
\def\bbX{{\mathbb{X}}}
\def\bbY{{\mathbb{Y}}}
\def\bbZ{{\mathbb{Z}}}

% Caligraphic capital letters
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}


\def\cd{\mathcal{d}}

% Sans serif capital letters
\def\sfA{\mathsf{A}}
\def\sfB{\mathsf{B}}
\def\sfC{\mathsf{C}}
\def\sfD{\mathsf{D}}
\def\sfE{\mathsf{E}}
\def\sfF{\mathsf{F}}
\def\sfG{\mathsf{G}}
\def\sfH{\mathsf{H}}
\def\sfI{\mathsf{I}}
\def\sfJ{\mathsf{J}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfM{\mathsf{M}}
\def\sfN{\mathsf{N}}
\def\sfO{\mathsf{O}}
\def\sfP{\mathsf{P}}
\def\sfQ{\mathsf{Q}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfU{\mathsf{U}}
\def\sfV{\mathsf{V}}
\def\sfW{\mathsf{W}}
\def\sfX{\mathsf{X}}
\def\sfY{\mathsf{Y}}
\def\sfZ{\mathsf{Z}}
\def\opt{\mathsf{OPT}}
\def\off{\mathsf{OFF}}
\def\rfl{\mathsf{RFL}}

% sans serif lowercase
\def\bydef{:=}
\def\sfa{{\mathsf{a}}}
\def\sfb{{\mathsf{b}}}
\def\sfc{{\mathsf{c}}}
\def\sfd{{\mathsf{d}}}
\def\sfee{{\mathsf{e}}}
\def\sfff{{\mathsf{f}}}
\def\sfg{{\mathsf{g}}}
\def\sfh{{\mathsf{h}}}
\def\sfi{{\mathsf{i}}}
\def\sfj{{\mathsf{j}}}
\def\sfk{{\mathsf{k}}}
\def\sfl{{\mathsf{l}}}
\def\sfm{{\mathsf{m}}}
\def\sfn{{\mathsf{n}}}
\def\sfo{{\mathsf{o}}}
\def\sfp{{\mathsf{p}}}
\def\sfq{{\mathsf{q}}}
\def\sfr{{\mathsf{r}}}
\def\sfs{{\mathsf{s}}}
\def\sft{{\mathsf{t}}}
\def\sfu{{\mathsf{u}}}
\def\sfv{{\mathsf{v}}}
\def\sfw{{\mathsf{w}}}
\def\sfx{{\mathsf{x}}}
\def\sfy{{\mathsf{y}}}
\def\sfz{{\mathsf{z}}}
\def\sf0{{\mathsf{0}}}

\def\1{{\bf 1}}
\def\N{{N}}
\def\Nt{{N_t}}
\def\Nr{{N_r}}
\def\Ne{{N_e}}
\def\Ns{{N_s}}
\def\Es{{E_s}}
\def\No{{N_o}}
\def\sinc{\mathrm{sinc}}
\def\dmin{d^2_{\mathrm{min}}}
\def\vec{\mathrm{vec}~}
\def\kron{\otimes}
\def\Pe{{P_e}}
\def\SINR{{\mathsf{SINR}}}
\def\SIR{{\mathsf{SIR}}}
\def\SNR{{\mathsf{SNR}}}
\def\MI{{\mathsf{MI}}}

\def\err{\textsf{err}} 

% Added by Takao
\def\nn{\nonumber}

% Chapter Numbers
\def\IntroChapter{Chapter 1}
\def\TCChapter{Chapter 2}
\def\MIMOChapter{Chapter 3}
\def\TWChapter{Chapter 4}
\def\CellularChapter{Chapter 5}
\def\MultiHopChapter{Chapter 6}
\def\PercolationChapter{Chapter 7}
\def\PWChapter{Chapter 8}
\def\TrCChapter{Chapter 9}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Robert's Notation Commands - Just temporary
\newcommand{\signb}{s} % not bold
\newcommand{\sig}{\mathbf{s}}
\newcommand{\Sig}{\mathbf{S}}
\newcommand{\noise}{\mathbf{v}}
\newcommand{\noisenb}{v}
\newcommand{\data}{\mathbf{y}}
\newcommand{\datanb}{{y}}
\newcommand{\Ff}{\mathsf{F}}
\newcommand{\ff}{\mathsf{f}}
\newcommand{\Hf}{\mathsf{H}}
\newcommand{\Gf}{\mathsf{G}}
\newcommand{\Ht}{\mathbf{H}}
\newcommand{\htime}{h}
\newcommand{\hfreq}{H}
\newcommand{\ftime}{f}
\newcommand{\ffreq}{F}
\newcommand{\Mt}{M_t}
\newcommand{\Mr}{M_r}
\newcommand{\evec}{\mathbf{e}}
\newcommand{\chanvec}{\mathbf{h}}
\newcommand{\symvecset}{\mathcal{S}}


%%%% Antonio's add %%%%%%%%%%%%%%%%%%%
\newcommand{\bLam}{\mathbf{\Lambda}}
\newcommand{\defeq}{\bydef}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\footrulewidth}{0pt}
\newcommand{\helv}{%
    \fontfamily{phv}\fontseries{b}\fontsize{9}{11}\selectfont}
\fancyhf{}
\fancyhead[LE,RO]{\helv  \thepage}
\newenvironment{dedication}
{
   \cleardoublepage
   \thispagestyle{empty}
   \vspace*{\stretch{1}}
   \hfill\begin{minipage}[t]{0.66\textwidth}
   \raggedright
}%
{
   \end{minipage}
   \vspace*{\stretch{3}}
   \clearpage
}


% Following should be included in each chapter's base.tex with
% appropriate chapter title.

%\fancyhead[RE]{\helv  \bfseries Advanced MIMO Communication}
%\fancyhead[LO]{\helv  \bfseries CHAPTER X. Spatial Multiplexing}


==> proof_lemma_switching_cost.tex <==
\section{Proof of Lemma \ref{lemma_switching_cost}}\label{app:lemma_switching}
	Using the triangle inequality followed by \(\norm{\u + \v} ^ {2} \leq 2 (\norm{\u}^{2} + \norm{\v}^{2})\) we obtain the following \(\forall t \geq 2\):
	\[
	\norm{\x_{t} - \x_{t - 1}} ^ {2}  \leq 2 \norm{\x_{t} - \bx^\star_{t - 1}} ^ {2} + 2 \norm{\x_{t - 1} - \bx^\star_{t - 1}} ^ 2  \leqtext{\eqref{one_fourth_0}} \frac{5}{2} \norm{\x_{t - 1} - \bx^\star_{t - 1}} ^ 2.
	\]
	Hence, the total switching cost of $\cA_o$ can be bounded by \begin{align}\nn
	\sum_{t = 1} ^ {T} \frac{1}{2} \norm{\x_{t} - \x_{t - 1}} ^ {2} &\stackrel{(a)}= \sum_{t = 2} ^ {T} \frac{1}{2}\norm{\x_{t} - \x_{t - 1}} ^ {2}, \\ &\stackrel{(b)}\leq \sum_{t = 1} ^ {T - 1} \frac{5}{2} \norm{\x_{t} - \bx_t^\star} ^ {2} ,\nn \\ &\leqtext{\eqref{actual_squared_bound}} 5 \norm{\x_{1} - \bx^\star_{1}} ^ {2} + 10 \P_{2, T} ^\star,	\nn				
	\end{align}
	where \((a)\) follows since \(\mathcal{A}_o\) chooses \(\x_{1} = \x_{0}\), \((b)\) follows from \(\norm{\x_{t} - \x_{t - 1}}^{2} \leq \frac{5}{2}\norm{\x_{t - 1} - \x_{t - 1}^\star}^{2}\). This completes the proof.

==> proof_of_lb_contraction.tex <==
\section{Proof of Lemma \ref{lb:contraction}}\label{ap:proof_lb_contraction}
If a deterministic online algorithm \(\cA\) chooses \(x_{1} \neq 0\) the adversary can choose \(f_{1}(x) = \frac{\mu}{2}x ^ {2}\). This makes \(\cA\) incur a non zero switching cost, while the \(\opt\) incurs zero cost. The competitive ratio is therefore unbounded. 

Next we consider the case when \(\cA\) chooses \(x_{1} = 0\). The adversary ends the game at \(T = 2\) and chooses to play the following functions: \(f_{1}(x) = \frac{\mu}{2}(x - \theta) ^ {2}\) where \(\theta > 0\) and \(f_{2}(x) = \frac{L}{2}x^{2}\). For this choice of functions, \(C_{\opt}\) can be upper bounded in the following manner:
\begin{align}\nn
	C_{\opt} = \min \sum_{t = 1} ^ {2} (f_{t}(x_{t}) + \abs{x_{t} - x_{t - 1}}) \leq 2\theta,
\end{align}
which follows by setting \(x_{1} = \theta\) and \(x_{2} = 0\) in the \(\opt\)'s minimization problem. 

The cost of \(\cA\) can be lower bounded by\begin{align}\nn
	C_{\cA} = \sum_{t = 1} ^ {2} \big(f_{t}(x_{t}) + \abs{x_{t} - x_{t - 1}}\big) = \frac{\mu}{2} \theta ^ {2} + \frac{L}{2} x_{2} ^ {2} + \abs{x_{2}}\geq \frac{\mu}{2} \theta ^ {2}.
\end{align}
The competitive ratio can thus be lower bounded by \[\mu_{\cA} = \frac{C_{\cA}}{C_{\opt}} \geq \frac{\mu}{4}\theta = \frac{\mu}{4} \frac{\cP_{2, T}^\star}{\cP_{T}^\star} = \Omega\bigg(\frac{\cP_{2, T}^\star}{\cP_{T}^\star}\bigg).\] This completes the proof.

==> proof_reduction.tex <==
\section{Proof of Lemma \ref{lem:reduction}}\label{proof_reduction}
Since \(\cA\) is not a contraction algorithm, there exists some \(t\) such that \(\abs{x_{t} - x_{t - 1} ^ \star} > \abs{x_{t - 1} - x_{t - 1} ^ \star}\). Let \(t = \tau\) be the smallest such time. So at time \(t = \tau\) we have \(\abs{x_{\tau} - x_{\tau - 1} ^ \star} > \abs{x_{\tau - 1} - x_{\tau - 1}^\star}\). First we consider the case when \(\tau > 2\). For times \(t\) that satisfy \(2 \leq t \leq \tau - 1\) we have \(\abs{x_{t} - x_{t - 1}^\star} \leq \abs{x_{t - 1} - x_{t - 1}^\star}\).  Consider the sequence of functions given by \(f_{1}(x) = \frac{\mu}{2}(x - \theta)^{2}\) where \(\theta > 0\) and \(f_{t}(x) = \frac{L}{2}x^{2}\) for \(2 \leq t \leq \tau\). Thus the adversary terminates the game at \(t = \tau\). Without loss of generality assume that \(x_{\tau - 1} \leq x_{\tau - 1} ^ \star = 0\). We have the following cases possible for the location of \(x_{\tau}\).
\begin{itemize}
	\item The case when \(x_{\tau} > - x_{\tau - 1}\). 
	Consider a contraction algorithm \(\cA^{'}\) that selects actions \(x_{1}^{'}, \ldots, x_{\tau} ^ {'}\) such that \(x_{t} = x_{t}^{'}\) for \(1 \leq t \leq \tau - 1\) and \(x_{\tau}^{'}\) in a manner such that \(\abs{x_{\tau}^{'} - x_{\tau - 1}^{\star}} \leq \abs{x_{\tau - 1}^{'} - x_{\tau - 1}^\star} \implies \abs{x_{\tau}'} \le \abs{x_{\tau - 1}^{'}}\). Clearly \(f_{\tau}(x_{\tau} ^ {'}) = \frac{L}{2} (x_{\tau}^{'})^{2} < \frac{L}{2}x_{\tau} ^ {2} = f_\tau(x_{\tau})\) and \(\abs{x_{\tau}^{'} - x_{\tau - 1}^{'}} = \abs{x_{\tau}^{'} - x_{\tau - 1}} < \abs{x_{\tau} - x_{\tau - 1}}\). Therefore we have \(\sum_{t = 1} ^ {\tau} \big(f_{t}(x_{t}) + \abs{x_{t} - x_{t  - 1}}) > \sum_{t = 1} ^ {\tau} \big(f_{t}(x_{t}^{'}) + \abs{x_{t}^{'} - x_{t - 1}^{'}}\big)\). This implies \(\mu_{\cA} \geq \mu_{\cA}^{'}\). The scenario is depicted in the following figure: 
	\begin{center}
		\begin{tikzpicture}
			\draw [gray, thick] (-6,0) -- (6,0);
			\filldraw[black] (-1,0) circle (1pt) node[anchor=north]{\(x_{\tau - 1}^\star = 0\)};
			\filldraw[black] (-4,0) circle (1pt) node[anchor=north]{\(x_{\tau - 1}\)};
			\filldraw[black] (3,0) circle (1pt) node[anchor=north]{\(-x_{\tau - 1}\)};
			\filldraw[black] (5,0) circle (1pt) node[anchor=north]{\(x_{\tau}\)};
			\filldraw[black] (1.5,0) circle (1pt) node[anchor=north]{\(x_{\tau}^{'}\)};
		\end{tikzpicture}
	\end{center}
	\item The case when \(x_{\tau} \leq x_{\tau - 1}\). There are 2 possible subcases depending on how far is \(x_{\tau}\) compared to \(x_{\tau - 1}\). 
	\begin{itemize}
		\item The subcase when \(2x_{\tau - 1} < x_{\tau} \leq x_{\tau - 1}\).  Consider a contraction algorithm that selects actions \(x_{1}^{'}, \ldots, x_{\tau}^{'}\) in such a way that \(x_{t} = x_{t} ^ {'}\) for \(1 \leq t \leq \tau - 1\) and \(x_{\tau} ^ {'}\) in a manner such that \(\frac{x_{\tau} ^ {'} + x_{\tau}}{2} = x_{\tau - 1} \implies x_{\tau} ^ {'} = 2x_{\tau - 1} - x_{\tau}\). This scenario is depicted in the following figure:
		\begin{center}
			\begin{tikzpicture}
				\draw [gray, thick] (-6,0) -- (6,0);
				\filldraw[black] (5,0) circle (1pt) node[anchor=north]{\(x_{\tau - 1}^\star = 0\)};
				\filldraw[black] (0,0) circle (1pt) node[anchor=north]{\(x_{\tau - 1}\)};
				\filldraw[black] (-5,0) circle (1pt) node[anchor=north]{\(2x_{\tau - 1}\)};
				\filldraw[black] (-2,0) circle (1pt) node[anchor=north]{\(x_{\tau}\)};
				\filldraw[black] (2,0) circle (1pt) node[anchor=north]{\(x_{\tau} ^ {'}\)};
			\end{tikzpicture}
		\end{center}
		We have \(\abs{x_{\tau} ^ {'} - x_{\tau - 1}^{'}} = \abs{x_{\tau - 1} - x_{\tau}}\), \(f_{\tau}(x_{\tau} ^ {'}) = \frac{L}{2}(x_{\tau}^{'}) ^ {2} < \frac{L}{2}x_{\tau} ^ {2} = f_{\tau}(x_{\tau})\). 
		So we have \(\sum_{t = 1} ^ {\tau}\big(f_{t}(x_{t}) + \abs{x_{t} - x_{t - 1}}\big) > \sum_{t = 1} ^ {\tau}(f_{t}(x_{t}^{'}) + \abs{x_{t}^{'} - x_{t - 1}^{'}}) \implies \mu_{\cA} \geq \mu_{\cA^{'}}\).
		\item The subcase when \(x_{\tau} \leq 2x_{\tau - 1}\). We consider the function \(g(x)\) defined as follows:
		\begin{align} \nn
			g(x) := \abs{x - x_{\tau - 1}} + \frac{L}{2}x ^ {2}
		\end{align}
		Since \(x_{\tau - 1} \leq 0\) by assumption, \(g(x)\) is a monotonically decreasing function over the interval \((-\infty, 2x_{\tau - 1}]\). So \(\min_{x \in (-\infty, 2x_{\tau - 1}]} g(x) = g(2x_{\tau - 1}) = 2L x_{\tau - 1} ^ {2} + \abs{x_{\tau - 1}}\). Since \(g(x)\) is a convex function in \(x\) we have \(\max_{x \in [x_{\tau - 1}, x_{\tau - 1}^\star]} = \max\{g(x_{\tau - 1}), g(x_{\tau - 1}^\star)\} = \max\{g(x_{\tau - 1}), g(0)\} = \max\{\frac{L}{2}x_{\tau - 1} ^ {2}, \abs{x_{\tau - 1}}\}\). So we have \(\min_{x \in (-\infty, 2x_{\tau - 1}]} g(x) > \max_{x \in [x_{\tau - 1}, x_{\tau - 1}^\star]}g(x)\). Therefore we have \(f_{\tau}(x_{\tau}) + \abs{x_{\tau} - x_{\tau - 1}} = g(x_{\tau}) > g(x_{\tau}' ) = f_{\tau}(x_{\tau} ^ {'}) + \abs{x_{\tau}^{'} - x_{\tau - 1}^{'}}\) for \(x_{\tau}^{'}\) selected by a contraction algorithm such that \(x_{\tau} ^ {'} \in [x_{\tau - 1}, x_{\tau - 1}^{\star}]\). Therefore we have \(\sum_{t = 1} ^ {\tau}\big(f_{t}(x_{t}) + \abs{x_{t} - x_{t - 1}}\big) > \sum_{t = 1} ^ {\tau}(f_{t}(x_{t}^{'}) + \abs{x_{t}^{'} - x_{t - 1}^{'}}) \implies \mu_{\cA} \geq \mu_{\cA^{'}}\). This scenario is depicted in the following figure:
		\begin{center}
			\begin{tikzpicture}
				\draw [gray, thick] (-6,0) -- (6,0);
				\filldraw[black] (4,0) circle (1pt) node[anchor=north]{\(x_{\tau - 1} ^ {\star} = 0\)};
				\filldraw[black] (1,0) circle (1pt) node[anchor=north]{\(x_{\tau - 1}\)};
				\filldraw[black] (-2,0) circle (1pt) node[anchor=north]{\(2x_{\tau - 1}\)};
				\filldraw[black] (-5,0) circle (1pt) node[anchor=north]{\(x_{\tau}\)};
			\end{tikzpicture}
		\end{center}
	\end{itemize}
\end{itemize}
It follows from Lemma \ref{lb:contraction} that the lower bound on \(\mu_{\cA ^ {'}}\) for the chosen functions is $\Omega(\frac{\mathcal{P}_{2, T} ^ \star}{\cP_{T} ^ \star})$. The proof for the case \(\tau = 2\) follows by the exact same arguments as above and are skipped for brevity. This completes the proof.

==> proof_total_cost_linear.tex <==
\section{Proof of Lemma \ref{up:omgd_linear}}\label{app:omgd_linear}We first bound the quantity \(\sum_{t = 1}^{T} \norm{\x_{t} - \x_{t}^\star}\) for \(\mathcal{A}_o\) as follows:
\begin{align}
	\sum_{t = 2} ^ {T} \norm{\x_{t} - \x_{t}^\star} & \stackrel{(a)}\leq \sum_{t = 2} ^ {T} \big(\norm{\x_{t} - \x_{t - 1}^\star} + \norm{\x_{t}^\star - \x_{t - 1}^\star}\big), \nn\\
	& \stackrel{(b)}\leq \sum_{t = 2} ^ {T} \frac{1}{2}\norm{\x_{t - 1} - \x_{t - 1}^\star} + \mathcal{P}_{T}^{\star}, \nn\\
	&= \frac{1}{2}\norm{\x_{1} - \x_{1}^\star} + \sum_{t = 2} ^ {T - 1} \frac{1}{2}\norm{\x_{t} - \x_{t}^\star} + \mathcal{P}_{T}^\star, \nn \\
	& \leq \frac{1}{2}\norm{\x_{1} - \x_{1}^\star} + \sum_{t = 2} ^ {T} \frac{1}{2}\norm{\x_{t} - \x_{t}^\star} + \mathcal{P}_{T}^\star, \nn,
\end{align}
where \((a)\) follows from the triangle inequality and \((b)\) follows from the contraction bound \eqref{one_fourth_0} attained by \(\mathcal{A}_{o}\). Rearranging, we obtain \begin{align}
	\sum_{t = 2} ^ {T} \norm{\x_{t} - \x_{t}^\star} \leq \norm{\x_{1} - \x_{1}^\star} + 2\mathcal{P}_{T}^\star \implies \sum_{t = 1} ^ {T} \norm{\x_{t} - \x_{t}^\star} \leq 2\norm{\x_{1} - \x_{1}^\star} + 2\mathcal{P}_{T}^\star. \label{cumulative_sum_cr_linear}
\end{align}
The overall switching cost of \(\cA_o\) can therefore be bounded as \begin{align*}
	\sum_{t = 1}^{T} \norm{\x_{t} - \x_{t - 1}} &\stackrel{(a)}= \sum_{t = 2}^{T} \norm{\x_{t} - \x_{t - 1}}, \\
	&\stackrel{(b)}\leq \sum_{t = 2}^{T}  \norm{\x_{t} - \x_{t - 1}  ^ \star} + \norm{\x_{t - 1} - \x_{t - 1} ^ \star}, \\
	&\stackrel{(c)}\leq \frac{3}{2} \sum_{t = 1}^{T - 1}\norm{\x_{t} - \x_{t}^\star}, \\
	&\stackrel{(d)}\leq 3\norm{\x_{1} - \x_{1}^\star} + 3\cP_{T}^\star,
\end{align*}
where \((a)\) follows since \(\x_{1} = \x_0\), \((b)\) follows from the Triangle inequality, \((c)\) follows from \eqref{one_fourth_0}, and \((d)\) follows from \eqref{cumulative_sum_cr_linear}, derived above. Finally, using the result of Lemma \ref{lemma_hitting_cost} to bound the total hitting cost \(\sum_{t = 1} ^ {T} f_{t}(\x_{t})\) completes the proof.
